A Concurrency-Optimal List-Based Set

Designing an efficient concurrent data structure is an important challenge that is not easy to meet. Intuitively, efficiency of an implementation is defined, in the first place, by its ability to process applied operations in parallel, without using unnecessary synchronization. As we show in this paper, even for a data structure as simple as a linked list used to implement the set type, the most efficient algorithms known so far are not concurrency-optimal: they may reject correct concurrent schedules. We propose a new algorithm for the list-based set based on a value-aware try-lock that we show to achieve optimal concurrency: it only rejects concurrent schedules that violate correctness of the implemented set type. We show empirically that reaching optimality does not induce a significant overhead. In fact, our implementation of the concurrency-optimal algorithm outperforms both the Lazy Linked List and the Harris-Michael state-of-the-art algorithms.

==> app-versioned.tex <==
\section{Versioned list algorithm}
\label{app:ver}
%
%
\subsection{Versioned trylock}
\label{sec:vertrylock}
%
\input{vlock-alg.tex}
%
The versioned try-lock is defined as %basically an encapsulation of 
a pair $\tup{\ms{ver}, \ms{lock}}$ of
a version number and a boolean locking state, 
%, which is simply a
%boolean, 
that can be modified together atomically.
The versioned try-lock (Algorithm~\ref{alg:vlock}) supports the following operations:
(1) $\lit{getVersion()}$: returns the current version. % associated to the specific pair.
(2) $\lit{tryLockAtVersion}(\ms{ver})$: tries to change the locking state from $\false$ to $\true$ atomically
if the current version number matches $\ms{ver}$.
The method fails and returns $\false$ if either the node is already locked or the version does not match; otherwise
it succeeds and returns $\true$.
(3) $\lit{lockAtCurrentVersion()}$: spins until it acquires the lock
with the current version. 
(4) $\lit{unlockAndIncrementVersion()}$: only called by the process that previously acquired the 
lock via successful $\lit{tryLockAtVersion}(ver)$ or $\lit{lockAtCurrentVersion()}$. It 
unconditionally sets the locking state from $\true$ to $\false$ and increments the current version number atomically
from $\tup{\ms{ver}, \true}$ to $\tup{\ms{ver}\text{+1}, \false}$. 

In our Java 8 implementation of the versioned try-lock
(Algorithm~\ref{alg:vlock}), we tested a single integer variable $\lit{AtomicInteger}$
that supports single-word CAS 
as well as the more recent
$\lit{StampedLock}$\footnote{\url{https://docs.oracle.com/javase/8/docs/api/java/util/concurrent/locks/StampedLock.html}}. 
A port of our list in C/C++ at  \url{https://goo.gl/IIVkCV} uses 
%One could alternately use 
the least significant bit of an unsigned integer on x86 architectures to represent the 
locking state where $0$ means ``unlocked'' and $1$ means ``locked''. 
Distinct version numbers are represented by all the even values: 
to extract the version we use a bit-mask that always sets the last bit
to $0$ when doing a bitwise \emph{and}.

\subsection{Versioned list description}
We now describe our versioned list implementation. 

\vspace{1em}\noindent\textbf{Contains.}
The algorithm for $\lit{contains}$ simply traverses in the
\emph{wait-free} manner, 
exactly as in the sequential algorithm
(Algorithm~\ref{alg:lists} of Appendix~\ref{app:seq}) except that in the end, 
we also check that $\ms{curr}$ is not deleted (Line~\ref{line:linr}). 
This wait-free traversal, introduced by Heller \emph{et al}.~\cite{HHL+05}, 
results in a highly efficient $\lit{contains}$ algorithm, as its only
overhead  (compared to the sequential implementation) 
comes from a single base object read, on $\ms{curr.deleted}$. 

\vspace{1em}\noindent\textbf{Pre-locking validation in insert and remove.}
For $\lit{insert}$ and $\lit{remove}$, 
we first traverse the list in a wait-free manner (Lines~\ref{line:traversal-start}--\ref{line:traversal-end}) 
%without any synchronization just like the sequential implementation 
until we find the position 
where a node might be inserted or deleted, i.e., where $\ms{prev.val} < v$ and $\ms{curr.val} \geq v$. 
%
Then we use the novel technique of \emph{pre-locking-validation}: 
it \emph{validates} the state of the nodes prior to locking. 
Generally, an optimistic lock-based algorithm follows this pattern for updates:
%
(1) read data on node,
(2) lock node,
(3) re-read \& validate integrity: if fail then unlock \& restart,
(4) modify data
(5) unlock node.

With pre-locking-validation, the new pattern becomes:
(1) read node version $ver$,
(2) read \& validate data integrity, if fail then restart,
(3) $\lit{try-lock-at-version}(ver)$: if fail then restart,
(4) modify data,
(5) $\lit{unlock-and-increment-version}$.
The reason why we can validate \emph{before} acquiring the lock
is that the consistency of the validation result is protected by the version number. 
% Observe that in this new pattern, any modification to the node first acquires a lock and the version is changed only
% when releasing the lock. 
% Thus, in case any concurrent thread is modifying or has modified the node between the read-version and 
% the try-lock-at-version steps, the try-lock will fail either because of a lock conflict or a new version number. 
%In contrast with sequence locks,  a writer does not need to increment twice the version per critical section.

\vspace{1em}\noindent\textbf{The validate function.}
The $\lit{validate}$  function
(Lines~\ref{line:validate-start}-\ref{line:validate-return}) 
%[[VG: rephrasing
invoked by our update operations is a short traversal that
%used by our update operations is
%basically a short versioned-traversal just like the wait-free one 
%except that it always reads and keeps the version of $\ms{prev}$ first, 
stores the version of $\ms{prev}$, then
checks that $\ms{prev}$ is not logically deleted and finally sets
$\ms{curr}$ to $\ms{prev.next}$. %\petr{the description is a bit unclear} 
%]]
%[[PK validate is only used by the update, ``necessary and sufficient''
%% seems out of place. 
%For our update operations, 
%the necessary and sufficient 
The validation conditions are 
%]]
(1) $prev$ is not deleted ($prev.deleted = \false$), and 
(2) $\ms{prev.next}$ points to $\ms{curr}$ ($\ms{prev.next = curr}$).  
% Observe that we do not need to check (3) $curr$ is not deleted 
% since the marking and unlinking of $curr$ happens in the critical section of $\lit{remove}$ 
% (Line~\ref{line:isdeleted} and Line~\ref{line:delcommit}). 
% Indeed, (1) and (2) imply (3): when an update operation holding the lock on $\ms{prev}$
% enters its \emph{critical section} (Line~\ref{line:inscommit} for $\lit{insert}$ and 
% Lines~\ref{line:isdeleted} and~\ref{line:delcommit} for $\lit{remove}$),
% if $\ms{curr.deleted}$ was set to $\true$, then $\ms{prev.next}$ 
% must have changed before $\lit{remove}$ exits the critical section. 

Note that after the traversal completes and before the validation starts, some new node could be inserted between 
$\ms{prev}$ and $\ms{curr}$ or $\ms{curr}$ could be deleted.
Instead of using the $\ms{curr}$ node from the traversal to check whether $\ms{prev.next} = \ms{curr}$
we simply re-traverse from the $\ms{prev}$ node.
%We do not use $\ms{curr}$ from the wait-free traversal to check $\ms{prev.next} = \ms{curr}$ because 
%concurrent threads could have inserted new nodes between $\ms{prev}$ and $\ms{curr}$ or 
%deleted $\ms{curr}$ before we start validate, so it's easier to just re-traverse from $\ms{prev}$. 
%[[[\textbf{SR: too long and sentence and does not seem to read well, especially the last line}]]]

During validation and locking, 
we might fail due to conflicts with a concurrent operation, 
in which case we need to abort and restart the operation. 
We included an optimization of \emph{partial abort} where instead of restarting from $\ms{head}$, 
we only need to restart from $\ms{prev}$ under the condition that $\ms{prev.deleted}$ is not $\true$
(we already know that $\ms{prev.val}<v$).  
As a result of this ``versioned-traversal'',  we get $\ms{prev}$ and
$\ms{curr}$ together with $\ms{prev}$'s version $pVer$ (Line~\ref{line:validate-return}): 
if the operation later successfully locks $\ms{prev}$ at $\ms{pVer}$,
we are sure that $\ms{prev}$ is not deleted and $\ms{prev.next = curr}$. 

\vspace{1em}\noindent\textbf{Inserting a node.}
For $\lit{insert}$, we create the new node \emph{before} entering the critical section (Line~\ref{line:new-node}): 
the reason here is that we want to optimize concurrency and minimize the length of the critical section. 
% Since no other threads can see the new node before we link it in (Line~\ref{line:inscommit}), 
% operations on the new node can be treated as local steps and there is no need to synchronize them. 
However, it is possible for our implementation to execute the node creation (Line~\ref{line:new-node}) 
multiple times since we could potentially abort later and restart. 
A possible optimization is to keep track of the $\ms{newNode}$ reference and make a check before Line~\ref{line:new-node} 
so that we allocate the memory at most once per $\lit{insert}$ operation. 
We enter the critical section by trying to lock $\ms{prev}$ at version $\ms{pVer}$ atomically in Line~\ref{line:inslock} ($pVer$ is the version
of the $\ms{prev}$ node obtained after validation in Line~\ref{line:insert-validate}).
If we obtain the lock successfully, it implies that we are already in a valid state (conditions (1) 
and (2) are satisfied). Once we have successfully acquired the lock on $\ms{prev}$, 
we link-in the new node (Line~\ref{line:inscommit}).

\vspace{1em}\noindent\textbf{Removing a node.}
For $\lit{remove}$, we also require the lock on $\ms{curr}$, which is obtained using the spin-lock in Line~\ref{line:spinlock}).
We need to lock $\ms{prev}$ at version $\ms{pVer}$ for the same reason as $\lit{insert}$:
to make sure no concurrent thread is inserting a node between $\ms{prev}$ and $\ms{curr}$ or 
deleting the $\ms{curr}$ node.
Additionally, we need to lock $\ms{curr}$ at its current version 
to prevent concurrent threads from inserting/deleting the node after $\ms{curr}$. 
Removing a node now involves two steps: a logical delete that sets $\ms{curr.deleted}$ to $\true$ (Line~\ref{line:isdeleted}) 
and a physical delete that changes $\ms{prev.next}$ (Line~\ref{line:delcommit}). 
% The logical deletion is non-trivial and very important 
% because it is the only \emph{local} indicator on a node itself that can tell us if the node is still in the list. 
% Without $\ms{curr.deleted}$ we have to back tract to check $\ms{prev.next}$ 
% but it will not work since $\ms{prev}$ could have been removed first then $\ms{curr}$ gets removed 
% (hence $\ms{prev}$ is still pointing to $\ms{curr}$ even though both have been removed). 
% This creates a recursive back tracking where to check whether $\ms{curr}$ has been removed, 
% we need to check $\ms{prev}$ first, and then the one before $\ms{prev}$ and so on. 

Finally, we exit the critical section by releasing the locks on the node(s) involved, increment 
the version in one atomic step (Line~\ref{line:relinsert}, \ref{line:curr-unlock}, \ref{line:relremove}) and 
return $\true$ for the operation. 

\input{pseudocode-2}
%
\subsection{Proof of correctness}
%
\begin{theorem}
\label{th:lr}
Versioned List is linearizable with respect to the $\ms{set}$ type.
\end{theorem}
\begin{proof}
%
Let $\alpha$ be a finite execution of Algorithm~\ref{alg:listver} and $<_\alpha$
denote the total-order on events in $\alpha$.
For the sake of the proof, we assume that $\alpha$ starts with an artificial
sequential execution of an insert operation $\pi_0$ that inserts $\ms{tail}$ and sets $\ms{head}.\ms{next}=\ms{tail}$. 
Let $H$ be the high-level history exported by $\alpha$.
%
%[[PK this does not appear in th main paper anymore
%Since \emph{linearizability} is a \emph{safety}
%property~\cite{Lyn96}, 
%it is sufficient for us to prove that every \emph{finite} high-level history $H$ is linearizable.
%]]

\vspace{0.8em}\noindent\textit{Completions.}
We obtain a completion $\tilde H$ of $H$ as follows.
The invocation of an incomplete $\lit{contains}$ operation is discarded.
The invocation of an incomplete $\pi=\lit{remove}$
operation that has not performed the write in Line~\ref{line:isdeleted} 
is discarded; otherwise, it is completed with response $\true$.
The invocation of an incomplete $\pi=\lit{insert}$
operation that has not performed the write in Line~\ref{line:inscommit} 
is discarded; otherwise, it is completed with response $\true$.

\vspace{0.8em}\noindent\textit{Linearization points.}
We obtain a sequential high-level history $\tilde S$ equivalent to $\tilde H$ by associating a linearization point $\ell_{\pi}$ 
with each operation $\pi$ as follows.
%
%\begin{itemize}
%\item 

For every $\pi=\lit{insert}(v)$ that returns $\true$ in $\tilde H$, $\ell_{\pi}$ is associated with 
%the last step of the \emph{tryCommit} (line~\ref{line:end-commit} of Algorithm~\ref{alg:elastic}) invoked in 
the write event in Line~\ref{line:inscommit} (rendering the node that
stores $v$ reachable from the \ms{head}); otherwise
$\ell_{\pi}$ is associated with the last $\lit{read}$ of a node's \emph{next} field performed by $\pi$ in $\alpha$. 

%\item
For every $\pi=\lit{remove}(v)$ that returns $\true$ in $\tilde H$, $\ell_{\pi}$ is associated with 
the write event in Line~\ref{line:isdeleted} (setting the
\ms{deleted} flag of a list's node); otherwise
$\ell_{\pi}$ is associated with the last $\lit{read}$ of a node's \emph{next} field performed by $\pi$ in $\alpha$. 

%\item
For $\pi=\lit{contains}(v)$ that returns $\true$, $\ell_{\pi}$
is associated with the last $\lit{read}$ performed by $\pi$ in which
$\pi$ finds the $\ms{deleted}$ field of a reachable node storing $v$ 
be $\false$ (Line~\ref{line:linr}).
%\item

For $\pi=\lit{contains}(v)$ that returns $\false$ in $H$, 
%
\begin{smallitemize}
\item
if $\pi$ reads $(X.value\neq v)$ in Line~\ref{line:linr}, where $X$ is the last node read by $\pi$ in $\alpha$,
$\ell_{\pi}$ is assigned to the read of the \emph{next} field of the node accessed by $\pi$ immediately before $X$
\item
if $\pi$ reads $(X.value = v)$ in Line~\ref{line:linr}, where $X$ is the last node read by $\pi$ in $\alpha$,
$\ell_{\pi}$ is defined as follows:
let $\pi_1$ be the $\lit{remove}$ operation that performs the last write
to $X.\ms{deleted}$ (Line~\ref{line:isdeleted}) prior to the read of $X.\ms{deleted}$ by $\pi$.
Then, $\ell_{\pi}$ is chosen to be the first event performed by $\pi_1$ immediately after the write to $X.\ms{deleted}$, but prior
the read of $X.\ms{deleted}$ by $\pi$. Otherwise if no such event of $\pi_1$ exists, then
$\ell_{\pi}$ is the read of $X.\ms{deleted}$ by $\pi$.
\end{smallitemize}
%
%\end{itemize}
%

Since linearization points are chosen within the intervals of 
operations performed in $\alpha$, for any two operations
$\pi_i$ and $\pi_j$ in ${\tilde H}$, if $\pi_i \rightarrow_{\tilde H}
\pi_j$, then $\pi_i \rightarrow_{\tilde S} \pi_j$.

We show that $\tilde S$ is consistent with the sequential specification of type \textit{set}.
When we refer to $\lit{read}(X)$, where
$X$ is a node, we mean the first read
of a node's field.

Let ${\tilde S}^k$ be the prefix of $\tilde S$ consisting of
the first $k$ complete operations. 
%(last event of ${\tilde S}^k$ is a response event).
%The state of the \emph{set} object at ${\tilde S}^0$ is $\emptyset$.
We associate each ${\tilde S}^k$ with a set $q^k$ of objects that were
successfully inserted and not subsequently successfully removed in ${\tilde S}^k$.
We show by induction on $k$ that the sequence of state transitions in
${\tilde S}^k$ is consistent with operations' responses in ${\tilde S}^k$ with respect to the \textit{set} type. 

%To prove that ${\tilde S}$ indeed consistent with \emph{set}, we
%proceed by induction on $k$. 
The base case $k=1$ is trivial: the \textit{tail} node containing
$+\infty$ is successfully inserted.
Suppose that ${\tilde S}^k$ is consistent with the \emph{set} type and
let $\pi_1$ with argument $v\in \mathbb{Z}$ and response $r_{\pi_{1}}$
be the last operation of ${\tilde S}^{k+1}$.  
We want to show that $(q^k,\pi_1,q^{k+1},r_{\pi_{1}})$ is consistent with the \textit{set} type. 
%We now prove that, upon the invocation of an operation $\pi_1$ with argument $v\in \mathbb{Z}$ applied at ${\tilde S}^k$ in state $q \in 2^{\mathbb{Z}}$,
%$(q,\pi_1,q',r_{\pi_{1}})$ is contained in the sequential
%specification of the \emph{set} type, where $q'$ is content of the
%\emph{set} object after ${\tilde S}^{k+1}$ defined in a natural way. We then say that ${\tilde S}^{k+1}$ satisfies $(q,\pi_1(v),q',r_{\pi_1})$.
%
%Let ${\tilde S}^k$ be the complete prefix of $\tilde S$ of length $k$.
%We proceed by induction on $k$.
%Let $\pi_1$ with argument $v\in \mathbb{Z}$ be the operation of the \emph{set} type applied at ${\tilde S}^k$ in state $q \in \mathbb{Z}$.
%

%\begin{enumerate}
\vspace{2mm}\noindent (1)
%\item[(1)]
Let $\pi_1=\lit{insert}(v)$ return $\true$ in ${\tilde S}^{k+1}$. 
We show below that each preceding $\pi_2=\lit{insert}(v)$ 
returning $\true$ is followed by $\lit{remove}(v)$ 
returning $\true$, such that
$\pi_2 \rightarrow_{{\tilde S}^{k+1}} \lit{remove}(v) \rightarrow_{{\tilde S}^{k+1}} \pi_1$.
Suppose the opposite. %by contradiction that such a $\pi_1$ and $\pi_2$ exist.
Observe that $\pi_1$ performs its penultimate $\lit{read}$ on a node $X$ 
that stores a value $v'<v$ and the last read is performed on a node that stores a value $v''>v$. 
%Clearly, $\pi_1$ also performs a $\lit{write}$ on $X$.
By construction of $\tilde S$, $\pi_1$ is linearized at the write on node $X$ in Line~\ref{line:inscommit}.
Observe that $\pi_2$ must also perform a $\lit{write}$ to the node $X$ 
(otherwise it is easy to see that one of $\pi_1$ or $\pi_2$ would return $\false$).
By assumption, the write to $X$ in shared-memory by $\pi_2$ in Line~\ref{line:inscommit} 
precedes the corresponding write to $X$ in
shared-memory by $\pi_1$. 
But $\pi_1$ can return $\true$ from the \emph{cas} performed in Line~\ref{line:inslock} only after 
$\pi_2$ releases the versioned lock on $X_1$ by performing the event in Line~\ref{line:relinsert}.
Thus, $\pi_1$ could not have returned $\true$---a contradiction.

Let $\pi_1=\lit{insert}(v)$ return $\false$ in ${\tilde S}^{k+1}$.
We show that there exists a preceding $\pi_2=\lit{insert}(v)$ returning 
$\true$ that is not followed by  $\pi_3=\lit{remove}(v)$ returning
$\true$, such that
$\pi_2 \rightarrow_{{\tilde S}^{k+1}} \pi_3 \rightarrow_{{\tilde S}^{k+1}} \pi_1$. 
Suppose that such a $\pi_2$ does not exist. Thus, $\pi_1$ must perform
its last $\lit{read}$ on a node $X$ that stores value $v''>v$, acquire the versioned lock on $X$ (Line~\ref{line:inslock})
and return $\true$---a contradiction to the assumption that $\pi_1$ returned $\false$.

It is easy to verify that the conjunction of the above two claims proves that 
$\forall q\in Q$; $\forall v\in \mathbb{Z}$, ${\tilde S}^{k+1}$ satisfies $(q,\lit{insert}(v),q \cup \{v\},(v \not\in q))$.

\vspace{2mm}\noindent (2)
%\item[(2)]
If $\pi_1=\lit{remove}(v)$, similar arguments as applied to $\lit{insert}(v)$ prove that 
$\forall q\in Q$; $\forall v\in \mathbb{Z}$, ${\tilde S}^{k+1}$ satisfies $(q,\lit{remove}(v),q \setminus \{v\},(v \in q))$.

\vspace{2mm}\noindent (3)
%\item[(3)]
Let $\pi_1=\lit{contains}(v)$ return $\true$ in ${\tilde S}^{k+1}$. 
We show that there exists $\pi_2=\lit{insert}(v)$ returning \emph{true} 
that is not followed by any $\lit{remove}(v)$ returning \emph{true}, such that
$\pi_2 \rightarrow_{{\tilde S}^{k+1}} \lit{remove}(v) \rightarrow_{{\tilde S}^{k+1}} \pi_1$.
Recall that $\pi_1$ is linearized at the last $\lit{read}$ of an node, say $X$, performed by $\pi$ when 
$\pi$ reads the $\ms{deleted}$ field
of $X$ to be $\false$ (Line~\ref{line:linr}). 
By the algorithm, 
%Lemma~\ref{lem:invar1}, 
there exists
$\pi_2=\lit{insert}(v)$ such that $\pi_2 \rightarrow_{{\tilde S}^{k+1}} \pi_1$ 
(let $\pi_2$ be the latest such operation).
Suppose that there exists a $\lit{remove}(v)$ that returns
\emph{true}, such that
$\pi_2 \rightarrow_{{\tilde S}^{k+1}} \lit{remove}(v) \rightarrow_{{\tilde S}^{k+1}} \pi_1$.
Thus, $\lit{remove}(v)$ performs the write event in Line~\ref{line:isdeleted} prior to the 
read of $X.\ms{deleted}$ by $\pi_1$. But then $\pi_1$ must read $X.\ms{deleted}$ to be $\true$
and return $\false$---a contradiction.

Now, let $\pi_1=\lit{contains}(v)$ return $\false$ in ${\tilde S}^{k+1}$. 
Thus, (1) there exists a $\pi_2=\lit{remove}(v)$ returning
\emph{true} that is not  
%$\lit{insert}(v) \rightarrow_{S} \lit{contains}(v)$ or 
followed by any $\lit{insert}(v)$ returning \emph{true},
such that 
$\pi_2 \rightarrow_{{\tilde S}^{k+1}} \lit{insert}(v) \rightarrow_{{\tilde S}^{k+1}} \pi_1$, or
(2) there does not exist any $\lit{insert}(v)$ returning $\true$ such that
$\lit{insert}(v) \rightarrow_{{\tilde S}^{k+1}} \pi_1$.
We consider two cases:
%
\begin{smallitemize}
\item 
Suppose that $\pi_1$ reads $(X.value \neq v)$ in Line~\ref{line:linr}, where $X$ is the last node read by $\pi_1$ in $\alpha$.
Thus, $\ell_{\pi_1}$ is assigned to the read of the \emph{next} field of the node, say $X'$ accessed by $\pi_1$ 
immediately before $X$.
Assume by contradiction that there exists
$\pi_2=\lit{insert}(v)$ that returns \emph{true} such that 
there does not exist any $\lit{remove}(v)$ that returns \emph{true}; 
$\pi_2 \rightarrow_{{\tilde S}^{k+1}} \lit{remove}(v) \rightarrow_{{\tilde S}^{k+1}} \lit{contains}(v)$.
But then $\pi_1$ must read $(X.value = v)$ in Line~\ref{line:linr} and return $\true$---contradiction.
\item
Suppose that $\pi_1$ reads $(X.value = v)$ and $X.\ms{deleted}$ to be $\true$ in Line~\ref{line:linr}.
Clearly, there exists a $\pi_2=\lit{remove}(v)$ that is concurrent to $\pi_1$ and returns $\true$ in ${\tilde H}$.
By the assignment of linearization points, $\ell_{\pi_1}$ is assigned to the first event performed
by $\pi_2$ immediately after the write to $X.\ms{deleted}$, but prior to the read of $X.\ms{deleted}$ by $\pi_1$, where $X$
is the last node read by $\pi_1$. 
We consider two cases:
(1) Suppose that some such event of $\pi_2$ exists.
We claim that there does not exist any $\pi_3=\lit{insert}(v)$ that returns $\true$ such that
$\pi_2 \rightarrow_{{\tilde S}^{k+1}} \pi_3 \rightarrow_{{\tilde S}^{k+1}} \pi_1$.
Any such $\pi_2$ must acquire the versioned lock on $X'$ (Line~\ref{line:inslock}), 
the node read by $\pi_1$ immediately prior to $X$. 
Since $\pi_1$ reads $(X.value = v)$ and $X.\ms{deleted}$ to be $\true$, $\pi_2$ must also acquire the versioned lock
on $X'$ (Line~\ref{line:remlock}). By our assumption, $\ell_{\pi_2} \rightarrow_{{\tilde S}^{k+1}} \ell_{\pi_3}$.
Thus, $\pi_3$ acquires the versioned lock on $X'$ only after $\pi_2$ releases it in Line~\ref{line:relremove}.
But we linearize $\pi_1$ prior to $\ell_{\pi_3}$ by choosing it to be the event performed by $\pi_2$
in Line~\ref{line:delcommit}---a contradiction to our assumption that $\ell_{\pi_3} <_{\alpha} \ell_{\pi_1}$.
(2)
Otherwise, if no such event of $\pi_2$ exists, $\ell_{\pi_1}$ is chosen as
the read of $X.\ms{deleted}$ by $\pi_1$. Since $\pi_2$ does not release the versioned lock on $X'$
prior to the read of $X.\ms{deleted}$ by $\pi_1$, there does not exist any $\lit{insert}(v)$ that returns $\true$
such that 
$ \lit{insert}(v) \rightarrow_{{\tilde S}^{k+1}} \pi_1$. Now, by the assignment of linearization points,
$\pi_2 \rightarrow_{{\tilde S}^{k+1}} \pi_1$.
\end{smallitemize}
%
%
%\end{enumerate}
%
Thus, inductively, the sequence of state transitions in ${\tilde S}$
satisfies the sequential specification of the \textit{set} type. 
\end{proof}
%
%
%
\begin{theorem}
\label{th:deadlock}
The versioned list provides deadlock-freedom.
\end{theorem}
%
\begin{proof}
%
Suppose that an update operation $\pi$ fails to return a matching response after taking infinitely many steps.
Intuitively, $\pi$ fails to do so because (1) it is returned $\bot$ from the call to $\lit{validate}$ in Line~\ref{line:insert-validate}
for $\lit{insert}$ (and resp. Line~\ref{line:delete-validate} for $\lit{remove}$), or (2)
it fails to acquire the lock on the $\ms{prev}$ node in Line~\ref{line:inslock} for $\lit{insert}$ 
(and resp. Line~\ref{line:remlock} for $\lit{remove}$),
or (3) it fails to acquire the lock on the $\ms{curr}$ node during Line~\ref{line:spinlock} by $\lit{remove}$.

In Case (1), there exists a concurrent $\lit{remove}$ operation that is executing the code
in its critical section and must eventually return the response $\true$.
In Case (2), if $\pi$ returns $\false$ from the call to $\ms{prev}.\lit{tryLockatVersion}$, then
some concurrent update operation has indeed succeeded to acquire the lock and enters its critical section
if its an $\lit{insert}$. Otherwise if this concurrent operation is a $\lit{remove}$, we are in Case (3)
i.e. $\lit{remove}$ does not return from the call to $\ms{curr}.\lit{lockAtCurrentVersion}$ in Line~\ref{line:spinlock}.
Thus, some other update operation has acquired the lock on the $\ms{curr}$ node of this $\lit{remove}$. Note that we can
iteratively extend this execution, but the last such process performing an update operation must eventually enter the critical
section and return a matching response.
\end{proof}
%


==> conc.tex <==
%!TEX root = paper-p.tex
\section{Concluding remarks}
\label{sec:conc}
%
Intuitively, the ability of an implementation to successfully process
interleaving steps of concurrent threads is an appealing property that
should be met by performance gains.
In this paper, we show support this intuition by presenting
concurrency-optimal list-based set that outperforms (less concurrent) 
state-of-the-art algorithms.        
Does the claim also hold for other data structures? We suspect so. For
example, similar but more general data structures, such as skip-lists
or tree-based dictionaries, may allow for optimizations similar to 
proposed in this paper. Exploring this is future work.     
%\petr{Some insights from the evaluation?}





==> exp-old.tex <==
%!TEX root = paper-p.tex
\section{Experimental evaluation}
\label{sec:eval}
%
We compared our versioned list in Java to the lock-based Lazy Linked List~\cite{HHL+05} and Harris-Michael's non-blocking 
list~\cite{harris-set,michael-set} with its wait-free and RTTI optimization suggested in Java by Heller et al.~\cite{HHL+05} using the Synchrobench benchmark suite~\cite{Gra15}.
%We conducted performance benchmarking of our Java implementation of Algorithm~\ref{alg:listver} 
%and compared it to the Lazy Linked list by Heller et al.~\cite{HHL+05} and Harris-Michael's non-blocking 
%list~\cite{harris-set,michael-set} with the wait-free $\lit{contains}$ optimization suggested by Heller et al.~\cite{HHL+05}. 
For the versioned list, we tested both a hand-crafted versioned lock and one implemented on top of the Java 8 StampedLock and only report the better results of the latter.
The source code is publicly available as part of Synchrobench at \url{https://github.com/gramoli/synchrobench/}.
%
\subsection{Results and evaluation}
We report the performance results of the three implementations obtained from x86 and SPARC architectures. 
Figures~\ref{fig:x86} and~\ref{fig:sparc} depict the number of operations per millisecond obtained on x86 and on SPARC, respectively.
We only report the results for a list size of $100$ on the SPARC architecture, 
since the curves on higher list sizes were similar for both architectures. 

The left column of both figures is the $\lit{contains}$-only workload, the right column is the update-only 
($\lit{insert}$ and $\lit{remove}$ only) workload, and the middle column is a more realistic workload with 90\% contains and 10\% updates. 
Note that the level of contention increases from bottom to top as the list size decreases 
(leading to a higher chance of concurrent threads accessing the same node) and 
left to right as the number of write operations increases. Also, since
each operation has 50\% chance to return $\false$, the
\emph{effective} updates are roughly half of the shown percentage. 

We also studied the contribution of  \emph{traversals} and
\emph{updates}  in the execution time used by $\lit{insert}$ and
$\lit{remove}$ in each algorithm.
The \emph{traversal} time is defined as the time between operation invocation and 
when it finds $prev$ and $curr$ where $prev.val < v \leq curr.val$ (including re-traversal time caused by abort and restart);
for our algorithm, we also include the time of $\lit{validate}$ function. 
The \emph{update} time is measured from just before locking to just after lock release; 
for Harris-Michael algorithm that does not use locks we simply
measured the time taken by the \emph{CAS} at the end of each update operation 
(excluding \emph{CAS}es that happen during list traversal). 
Table~\ref{tab:traversal} shows the relative execution time per operation per thread normalized by the lowest number among the data (shaded cell). 

% Observation 1: Our alg outperforms others
We can see that our new list algorithm outperforms both Harris-Michael's and the Lazy Linked List algorithms and 
remains scalable even under extremely heavy contention (the top-right corner of the throughput graphs). 
The only place where our algorithm drops in performance is when 
there are more threads than cores (above $64$ threads, ``core-saturation'')
and contention is high.
This is an inherent problem to all lock-based algorithms: 
a thread holding a lock gets preempted from the CPU, 
while any other thread contending on the same lock cannot make progress 
even if it  is assigned the CPU time. 
(We can see this from Table~\ref{tab:traversal} that at 72 threads our update in the critical section took more than 100\% longer than 64 threads.)

% Observation 2: problem with HM
\vspace{1em}\noindent\textbf{Comparison against Harris-Michael.} 
Harris-Michael's algorithm in general scales well and performs really
well under high contention and core saturation (at 72 threads). 
This can be explained by the fact that the algorithm is nonblocking: a thread preempted from the CPU at any time does 
not indefinitely hamper the progress of other threads. 

%[[VG: no longer up-to-date
%However, we noticed that even though all the three algorithms use exactly the same wait-free $\lit{contains}$ algorithm, 
%Harris-Michael's optimized $\lit{contains}$ is slower than the other two. 
%This might be explained by the extra indirection in reading the $\ms{next}$ pointer from the 
%combined \emph{pointer-plus-boolean} when traversing each node (we implemented this 
%using the \textsf{AtomicMarkableReference} in \textsf{java.util.concurrent.atomic} package). 
%From the $\lit{contains}$-only graphs in the left column, 
%we can see that the list traversal of Harris-Michael using $\ms{node.next.getReference}()$ is approximately $50\%$ 
%slower compared to simply reading the next node reference using $node.next$ in the other two algorithms. 
%
%%[[PK play down a bot
%%We believe that there should 
%There might 
%%]]
%exist a more efficient way to implement the atomic \textit{compare-and-swappable-pointer-plus-boolean} 
%construct used by Harris-Michael's algorithm than Java's \textsf{AtomicMarkableReference}.  In an unmanaged language for example, 
%the inherent redirections of \textsf{AtomicMarkableReference} could
%potentially be avoided with $\lit{sun.misc.Unsafe}$ 
%to use a bitmask on a memory address, however, this is not recommended in Java.
%%However, some inherent overhead should be there. Intuitively, reading a pointer from a combined \textit{pointer-plus-boolean} should be more expensive than reading a standalone pointer because of the added complexity. \petr{What added complexity?}\textcolor{red}{(Di: maybe removed this paragraph to save space?)}
%]]
We can see, however, on the left-hand side of the Figures~\ref{fig:x86} and~\ref{fig:sparc} that even though the three algorithms 
feature the wait-free $\lit{contains}$ algorithm, our implementation of the Harris-Michael's $\lit{contains}$ is slower than the other two.
The reason is the extra indirection needed when reading the $\ms{next}$ pointer in the combined \emph{pointer-plus-boolean} structure.
Note that the original C-like pseudocode of Harris~\cite{harris-set} suggested the architecture-specific use of a bitmask on x86. 
While we could have done so in Java using $\lit{sun.misc.Unsafe}$ this is 
not recommended at it may annihilate the portability of the implementation. To avoid the overhead of reading an extra field when fetching the Java $\lit{AtomicMarkableReference}$
we implemented the run-time type identification (RTTI) variant with two subclasses that inherit from a parent node class and that represent the marked and unmarked 
states of the node as previously suggested~\cite{HHL+05}. 
This optimization requires, on the one hand, that a $\lit{remove}$ casts the subclass instance to the parent class to create a corresponding node in the marked state. It allows, on the other hand, the traversal to simply check the mark of each node by simply invoking $\lit{instanceof}$ on it to check the subclass the node instantiates. 
%Our first attempt was to use the simplified variant of Harris-Michael in Java~\cite{HS08} invoking $\lit{getReference}$ that requires an extra read to return the 
%reference of a node. 

From Table~\ref{tab:traversal} we can see that Harris-Michael's algorithm has the most efficient updates because it only 
uses \emph{CAS}, however it spends much longer on list traversal. 
We also found that above $40$ threads, there is around $5\%$ 
of the traversal time under 100\% update workloads that is spent on attempts to unlink marked nodes during the traversal. 

\vspace{1em}\noindent\textbf{Comparison against the Lazy Linked List.}  
The Lazy Linked List has almost the same performance as our algorithm under low contention 
(the left column and the bottom row in the graphs) because both share the same wait-free list traversal with 
zero overhead (as the sequential code does) and for the updates, 
when there is no interference from concurrent operations, 
the difference between our pre-locking-validation and Heller's post-locking-validation becomes negligible. 

The difference raises however as the contention appears.
%However, as contention increases, 
The performance of the Lazy Linked List drops significantly due to its intense lock competition (as briefly explained in Section~\ref{sec:intro}). 
By contrast, there are several features in our implementation that reduce the amount of contention on the locks 
significantly. 
For example, the pre-locking-validation that uses the versioned try-lock avoids aborting once the lock is acquired: 
if we cannot acquire the try-lock immediately 
because either the version has changed (meaning some concurrent thread has just modified the node) or the node is already locked 
(which means the version is going to change when it is unlocked), 
then we can already restart and try to read the new version. 
%[[[\textbf{SR: this is not true for the second lock during remove right?}]]] [[[VG: I guess it is true only for the the try-lock]]]
%[[PK already said that we do not abort once grab the (first) lock
%Once the first try-lock is acquired, the $\lit{remove}$ operation may
%spin to acquire a second lock that we know will eventually get
%released (in the absence of failure).
%]]
%\textcolor{red}{(Di: in our latest algorithm if the first try-lock on prev succeed then the operation is guaranteed to succeed and can no longer abort)}
Another feature is that our $\lit{insert}$ and $\lit{remove}$ operations check 
the node value before locking so in case the update fails (because the value is present or absent),
it returns with no particular overhead compared to $\lit{contains}$. 
Table~\ref{tab:traversal} shows the tremendous increase in execution time for the Lazy Linked List because of the contention on locks. 


%We also performed broken down execution time analysis on different parts of our implementation (cf. Table~\ref{tab:traversal}).
%


==> extras.tex <==
\begin{proof}
%
Let $\alpha$ be a finite execution of \name implementation and $<_\alpha$
denote the total-order on events in $\alpha$.
For the sake of the proof, we assume that $\alpha$ starts with an artificial
sequential execution of an insert operation $\pi_0$ that inserts $\ms{tail}$ and sets $\ms{head}.\ms{next}=\ms{tail}$. 
Let $H$ be the high-level history exported by $\alpha$.
Since \emph{linearizability} is a \emph{safety}
property~\cite{Lyn96}, 
it is sufficient for us to prove that every \emph{finite} high-level history $H$ is linearizable.

\vspace{0.8em}\noindent\textit{Linearization points.}
We obtain a sequential high-level history $\tilde S$ equivalent to $\tilde H$ (We obtain a completion $\tilde H$ is a completion of of $H$) by associating a linearization point $\ell_{\pi}$ 
with each operation $\pi$ as follows.
%
%\begin{itemize}
%\item 

For every $\pi=\lit{insert}(v)$ that returns $\true$ in $\tilde H$, $\ell_{\pi}$ is associated with 
%the last step of the \emph{tryCommit} (line~\ref{line:end-commit} of Algorithm~\ref{alg:elastic}) invoked in 
the write event in Line~\ref{line:reach} (rendering the node that
stores $v$ reachable from the \ms{head}); otherwise
$\ell_{\pi}$ is associated with the last $\lit{read}$ of a node's \emph{next} field performed by $\pi$ in $\alpha$. 

%\item
For every $\pi=\lit{remove}(v)$ that returns $\true$ in $\tilde H$, $\ell_{\pi}$ is associated with 
the write event in Line~\ref{remove:deleted} (setting the
\ms{deleted} flag of a list's node); otherwise
$\ell_{\pi}$ is associated with the last $\lit{read}$ of a node's \emph{next} field performed by $\pi$ in $\alpha$. 

%\item
For $\pi=\lit{contains}(v)$ that returns $\true$, $\ell_{\pi}$
is associated with the last $\lit{read}$ performed by $\pi$.
%\item

For $\pi=\lit{contains}(v)$ that returns $\false$ in $H$, 
%
\begin{smallitemize}
\item
if $\pi$ reads $(X.val\neq v)$ in Line~\ref{line:linrl}, where $X$ is the last node read by $\pi$ in $\alpha$,
$\ell_{\pi}$ is assigned to the read of the \emph{next} field of the node accessed by $\pi$ immediately before $X$
\item
if $\pi$ reads $(X.val = v)$ in Line~\ref{line:linrl}, where $X$ is the last node read by $\pi$ in $\alpha$,
$\ell_{\pi}$ is defined as follows:
let $\pi_1$ be the $\lit{remove}$ operation that performs the last write
to $X.\ms{deleted}$ (Line~\ref{remove:deleted}) prior to the read of $X.\ms{deleted}$ by $\pi$.
Then, $\ell_{\pi}$ is chosen to be the first event performed by $\pi_1$ immediately after the write to $X.\ms{deleted}$, but prior
the read of $X.\ms{deleted}$ by $\pi$. Otherwise if no such event of $\pi_1$ exists, then
$\ell_{\pi}$ is the read of $X.\ms{deleted}$ by $\pi$.
\end{smallitemize}
%
%\end{itemize}
%

Since linearization points are chosen within the intervals of 
operations performed in $\alpha$, for any two operations
$\pi_i$ and $\pi_j$ in ${\tilde H}$, if $\pi_i \rightarrow_{\tilde H}
\pi_j$, then $\pi_i \rightarrow_{\tilde S} \pi_j$.
%

Let ${\tilde S}^k$ be the prefix of $\tilde S$ consisting of
the first $k$ complete operations. 
%(last event of ${\tilde S}^k$ is a response event).
%The state of the \emph{set} object at ${\tilde S}^0$ is $\emptyset$.
We associate each ${\tilde S}^k$ with a set $q^k$ of objects that were
successfully inserted and not subsequently successfully removed in ${\tilde S}^k$.
We show by induction on $k$ (via a case-by-case analysis) that the sequence of state transitions in
${\tilde S}^k$ is consistent with operations' responses in ${\tilde S}^k$ with respect to the \textit{set} type. 

\vspace{0.8em}\noindent\textit{Deadlock freedom.} The only nontrivial case to analyse here is the case of update operations. Suppose that an update operation $\pi$ fails to return a matching response after taking infinitely many steps. However, in this case, it implies that there exists a concurrent $\lit{insert}$ or $\lit{remove}$ operation that successfully acquires the lock and completes its operation, thus implying deadlock-freedom.
%
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
%
Take any schedule $\sigma$ of the \name implementation. 
Theorem~\ref{th:linearizable-list} implies that the high-level history of $\sigma$
is linearizable with respect to the \emph{set} type.  
% By inspecting the pseudo-code, we
% observe that no write event is aborted. Thus, in $\sigma$,
% every read operation returns the last written value.   

To show our algorithm is locally serializable, we first remark that every operation
traverses the list starting from the $\ms{head}$ node and reads the
$\ms{next}$ field of a node to locate the subsequent node.  
Before adding a new node to the list (Lines~\ref{insert:creation:1} and \ref{insert:creation:2}),
each $\lit{insert}$ operation initializes the node's $\ms{val}$ and $\ms{next}$ field, so that    
at all times the $\ms{next}$ field of a node 
stores a pointer to  an inserted node with a strictly higher  value or
to the $\ms{tail}$ node.
Furthermore, the values stored in the list are integers, every
operation invoked with parameter $v$ eventually locates the node
storing $v$ or a higher value. 
Thus, every sequence of non-aborted
events of every operation $\pi$ is finite.
Hence, there exists a sequence of insert
operations $S_0$, such that $S_0\cdot\sigma|\pi$ is a sequential
schedule of {\LL}.         

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Proof sketch}\\
Let $\sigma$ be any schedule of our concurrent implementation. For every update operation $\pi$ in $\sigma$, $\sigma|\pi$ is defined to be the subsequence
$\sigma|\pi$ consisting of the reads, writes and node creation events from the last
invocation of the function $\lit{waitfreeTraversal}$ by $\pi$ in Lines~\ref{insert:restart} and \ref{remove:restart}; and
for every $\pi=\lit{contains}$ in $\sigma$, $\sigma|\pi$ is the subsequence
$\sigma|\pi$ consisting of the reads and writes on a node's \emph{val} and \emph{next} fields.

\vspace{0.8em}\noindent\textit{\name accepts every observably correct schedule.}
We argue that any schedule \emph{rejected} by our algorithm is  
not observably correct.
More precisely, we show that an operation restarts a fragment
of it execution (in Lines~\ref{insert:restart}, \ref{remove:restart}) 
only if extending it with a read or a write
on $\ms{next}$ or $\ms{val}$ fields would result in schedule that is
not observably correct.

We first observe that if a node is logically deleted
(Line~\ref{remove:deleted}), then its next write renders the node
unreachable from the \ms{head} node. 
Thus, an update operation $\pi$ partially restarts because of reading a logically
deleted node (Lines~\ref{insert:restart},
or \ref{remove:restart}) only if it is concurrent with a
\lit{remove} operation which, when completed would physically remove
the node addressed by $\pi$ at the end of its traversal. 
It is easy to see that regardless of what this operation $\pi$ is
($\lit{insert}(v)$ or $\lit{remove}(v)$), if we complete it in turn
and then extend the resulting schedule with $\lit{contains}(v)$, the
effect of $\pi$ will not be seen and the schedule will not be
linearizable.

Similarly, an update operation $\pi$ partially restarts (in Line~\ref{insert:check} for $\lit{insert}$ and Lines~\ref{remove:check:prev} and \ref{remove:check:curr} for $\lit{remove}$) 
after finishing its traversal phase, if
it fails in grabbing a lock on one of the nodes it is about to modify.
Thus, $\pi$ is concurrent with another update operating on the same node.  
Again, by completing both $\pi$ and the concurrent update, we obtain a
schedule in which one of the updates is ``lost'', so that its
extension with some $\lit{contains}(v)$ will not be linearizable with respect to the set specification.                



==> hohAlgo.tex <==
\begin{algorithm*}[t]
\caption{Pessimistic lock-based implementation $I^{H}$ of the list-based set}
\label{alg:listc}
  \begin{algorithmic}[1]
  	\begin{multicols}{3}
  	{\size
	
	\Part{Shared variables}{
		\State Initially $\ms{head}$, $\ms{tail}$,
		\State ~~~$\ms{head}.val=-\infty$, 
		\State ~~~$\ms{tail}.val=+\infty$,
		\State ~~~$\ms{head}.next=\ms{tail}$
	}\EndPart
	
	
	\Statex
	
	\Part{$\lit{insert}(v$)}{
		\State $\lit{lock}(\ms{head})$ 
		\State $\ms{new} \gets \lit{read}(\ms{head})$
		\State $\ms{curr} \gets \ms{head}$
		%\State $\ms{new} \gets \ms{old}$
%		\If{($\lit{read}(\ms{prev.val})=s\vee$
%			\State ~~~~~~$\ms{prev} = \ms{Tail})$}
%			\State $\ms{result} \gets \lit{false}$
%			\State $\lit{goto}$ Line~\ref{line:release}
%		\EndIf
		%\State $\ms{curr} \gets \lit{read}(\ms{prev.next})$ 
%	   	\While{$(\ms{\lit{read}(curr.val)} < (s) \vee$
%			\State ~~~~~~$\ms{curr} \neq \ms{Tail})$} 
		\While{$\ms{new.val} < v$}
			\State $\ms{prev} \gets \ms{curr}$
			\State $\ms{old} \gets \ms{new}$
			\State $\ms{curr} \gets  \ms{new.next}$
			\State $\ms{new}\gets \lit{read}(\ms{curr})$
 	  	\EndWhile
		\If{$\ms{new.val} \neq s$} \label{line:aif}
			\If{$\ms{prev}\neq \ms{head}$}			
				\State $\lit{lock}(\ms{prev})$ \label{line:aei}
			\EndIf		
			\State $X \gets \lit{new-node}(v,\ms{curr})$ \label{line:new}
			%\State $X.\ms{next} \gets \ms{curr}$ \label{line:nafter}
			\State $\lit{write}(\ms{prev}, [\ms{old.val},X])$ \label{line:nadd}
			%\State $\ms{result} \gets \lit{true}$
		%\Else{} $\ms{result} \gets \lit{false}$
		\EndIf
		\If{$\ms{prev}\neq \ms{head}$}
			\State $\lit{unlock}(\ms{prev})$
		\EndIf
		%\State $\lit{release}(\ms{curr})$ \label{line:release}	
		\State $\lit{unlock}(\ms{head})$
		\Return $(\ms{new.val} \neq v)$	\EndReturn
    	}\EndPart
	
	\newpage
	
	
	  \Part{$\lit{contains}(v$)}{
		\State $\lit{lock}^S(\ms{head})$
		\State $\ms{new} \gets \lit{read}(\ms{head})$
		\State $\ms{curr} \gets \ms{head}$
		%\State $\ms{new} \gets \ms{old}$
		%\State $\ms{curr}\gets  \lit{read}(\ms{prev.next})$
		\While{$\ms{new.val} < v$} \label{line:read}
				%\State $\lit{release}(\ms{prev})$
				\State $\ms{prev}\gets \ms{curr}$
				\State $\ms{old} \gets \ms{new}$
				\State $\ms{curr}\gets \ms{new.next}$
				\State $\lit{lock}^S(\ms{curr})$
				\State $\ms{new}\gets \lit{read}(curr)$
				\State $\lit{unlock}(\ms{prev})$
 	    \EndWhile
%		\If{$\ms{t.val} = v$} \label{line:check}
% 	   		\State $\ms{result}\gets \lit{true}$
%		\Else{} $\ms{result} \gets \lit{false}$
% 	   	\EndIf
 	   	\State $\lit{unlock}(\ms{curr})$
 	   	%\State $\lit{release}(\ms{curr})$
 	   	\Return $(\ms{new.val} = v)$ \EndReturn \label{line:check}
   	 }\EndPart
   	 
	 \newpage
	  \Part{$\lit{remove}(v$)}{
		\State $\lit{lock}(\ms{head})$ 
		\State $\ms{new} \gets \lit{read}(\ms{head})$
		\State $\ms{curr} \gets \ms{head}$
		%\State $\ms{new} \gets \ms{old}$
%		\If{($\lit{read}(\ms{prev.val})=s\vee$
%			\State ~~~~~~$\ms{prev} = \ms{Tail})$}
%			\State $\ms{result} \gets \lit{false}$
%			\State $\lit{goto}$ Line~\ref{line:release2}
%		\EndIf
		%\State $\ms{curr}\gets  \lit{read}(\ms{prev.next})$ 
 	   	\While{$\ms{new.val} < v$}
			\State $\ms{prev} \gets \ms{curr}$
			\State $\ms{old} \gets \ms{new}$
			\State $\ms{curr} \gets  \ms{new.next}$
			\State $\ms{new}\gets \lit{read}(\ms{curr})$
 	  	\EndWhile
 	   	\If{$\ms{new.val} = v$} \label{line:dif}
 	   		\If{$\ms{prev}\neq \ms{head}$}
				\State $\lit{lock}(\ms{prev})$ \label{line:aer}
			\EndIf
 	    	\State $\lit{lock}(\ms{curr})$
			\State $\lit{write}(\ms{prev}, [\ms{old.val},\ms{new.next}])$  \label{line:remove1}
			\State $\lit{write}(\ms{curr}, [\bot,\bot])$  \label{line:remove2}
%			\State $\ms{result} \gets \lit{true}$
%		\Else{} $\ms{result} \gets \lit{false}$
		\If{$\ms{prev}\neq \ms{head}$}		
			\State $\lit{unlock}(\ms{prev})$ 
		\EndIf
		\State $\lit{unlock}(\ms{curr})$ \label{line:release2}
		\EndIf
		\State $\lit{unlock}(\ms{head})$
		\Return $(\ms{new.val} = v)$ \EndReturn
   	}\EndPart
	 
%   	 \Part{spin-lock(\ms{X}, \ms{mode})}{
%   	 	\State $\ell \gets \lit{false}$
%		\While{$\neg \ell$} 
%			\State $\ell \gets \lit{acquire}^{\ms{mode}}(X)$
% 	   	\EndWhile
%	}\EndPart
	
	}
	\end{multicols}

  \end{algorithmic}
\end{algorithm*}


==> list-new.tex <==
%!TEX root = paper-p.tex
%\subsection{Proof of linearizability}
%\label{sec:correct}
%

==> ll-alg.tex <==
\begin{algorithm*}[ht]
\caption{Optimistic implementation {$I^L$} (\textit{sorted linked list}) of \emph{set} type}
\label{alg:lists}
  \begin{algorithmic}[1]
  	\begin{multicols}{2}
  	{\size
	
	\Part{Shared variables}{
		\State Initially $\ms{head}$, $\ms{tail}$,
		\State ~~~$\ms{head}.val=-\infty$, $\ms{tail}.val=+\infty$
		\State ~~~$\ms{head}.next=\ms{tail}$
	}\EndPart
	
	\Statex
	
	\Part{$\lit{insert}(v$)}{
                \State $\ms{old} \gets \ms{head}$  		 			\Comment{copy the address for the potential write}
		\State $\ms{prev} \gets \lit{read}(\ms{head})$  			\Comment{fetch the head node struct from memory}
		\State $\ms{curr} \gets \lit{read}(\ms{prev.next})$		\Comment{the next element is stored locally}
		\If{\ms{curr.marked}}
		  \Return $(\ms{curr.val}=v)$ \EndReturn
		\EndIf
		\While{$\ms{curr.val} < v $}
                \Comment{If the current value is less than $v$}
                       \State $\ms{old} \gets \ms{prev.next}$  \Comment{pointer to the next element}
			\State $\ms{prev} \gets \ms{curr}$ 				\Comment{move on}
%			\State $\ms{curr}\gets \ms{new}$
%			\State $\ms{curr} \gets \ms{new.next}$
			\State $\ms{curr} \gets \lit{read}(\ms{curr.next})$ 	\Comment{fetch from memory}
		\EndWhile
		\If{$\ms{curr.val} \neq v$}							\Comment{val is stored locally}
			\State $X \gets \lit{new-node}(v,\ms{prev.next})$ 	\Comment{value v and address of curr}
%			\State $\lit{write}(\ms{prev},[\ms{old.val},X])$ 	
			\State $\lit{write}(\ms{old}, [\ms{prev.val},X])$ 	\Comment{stores val and next field pointing to X}
		\EndIf
		\Return $(\ms{curr.val}\neq v)$ 						\Comment{re-evaluate same condition}\EndReturn
   	}\EndPart
	
	\newpage
	
	\Part{$\lit{remove}(v$)}{

	        \State $\ms{old} \gets \ms{head}$  					\Comment{copy the address for the potential write}
		\State $\ms{prev} \gets \lit{read}(\ms{head})$  			\Comment{fetch the head node struct from memory}
		\State $\ms{curr} \gets \lit{read}(\ms{prev.next})$ 		\Comment{the next field is stored locally}
		\While{$\ms{curr.val} < v $} 	
					\Comment{the val field is stored locally}
                       \State $\ms{old} \gets \ms{prev.next}$
                       \Comment{pointer to the next element}
			\State $\ms{prev} \gets \ms{curr}$ 				\Comment{move on}
%			\State $\ms{curr}\gets \ms{new}$
%			\State $\ms{curr} \gets \ms{new.next}$
			\State $\ms{curr} \gets \lit{read}(\ms{curr.next})$ 	\Comment{fetch from memory}
		\EndWhile
		\If{$\ms{curr.val} = v$}							\Comment{val is stored locally}
%			\State $\lit{write}(\ms{prev} ,[\ms{old.val},\ms{new.next}])$
			\State $\lit{write}(\ms{old},
                               [\ms{prev.val},\ms{curr.next}])$
                               \Comment{next field pointing to curr.next}
		\EndIf
		\Return $(\ms{curr.val}=v)$ 						\Comment{re-evaluate same condition}\EndReturn	
   	}\EndPart
	
	\Statex
	
	\Part{$\lit{contains}(v$)}{
		\State $\ms{prev} \gets \lit{read}(\ms{head})$  			\Comment{fetch the head node struct from memory}
		\State $\ms{curr} \gets \lit{read}(\ms{prev.next})$
				\Comment{the next field is stored locally}
		\If{\ms{curr}.marked}
		  \Return $\bot$ \EndReturn
 		\EndIf
		\While{$\ms{curr.val} < v $} 						\Comment{the val field is stored locally}
			\State $\ms{prev} \gets \ms{curr}$ 				\Comment{move on}
%			\State $\ms{curr}\gets \ms{new}$
%			\State $\ms{curr} \gets \ms{new.next}$
			\State $\ms{curr} \gets \lit{read}(\ms{curr.next})$ 	\Comment{fetch from memory}
		\EndWhile
 	   	\Return $(\ms{curr.val}=v)	$						\Comment{val is stored locally}\EndReturn
   	 }\EndPart

		
	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm*}


==> optimal-proof-versionedlist.tex <==
\subsection{Optimal concurrency of the Versioned List}
%
In this section, we prove that the versioned list accepts practically every correct interleaving of the sequential code.
Specifically, we show that any finite schedule rejected by our algorithm  is not \emph{observably correct}. 
A correct schedule $\sigma$ is observably correct
if by completing update operations in $\sigma$ and 
extending, for any $v\in \mathbb{Z}$, the resulting schedule with a complete sequential execution 
$\lit{contains}(v)$, applied to the resulting contents of the list,
we obtain a correct schedule.
Here the contents of the list after a given correct schedule 
is determined based on the order of its write operations. For each
node, we define the resulting state of its
\textit{next} field based on the last write in the schedule. 
Since in a correct schedule each new node is first created and then
linked to the list, we can reconstruct the \emph{state of the list} by
iteratively traversing it, starting from $\ms{head}$.    
 
Intuitively, a schedule is observably correct if it incurs no ``lost updates''.
Consider, for example a schedule (cf. Figure~\ref{fig:ex1}) in which two operations,
$\lit{insert}(1)$ and $\lit{insert}(2)$ applied to the initial empty
set. Imagine that they first both read $\ms{head}$, then both read
$\ms{tail}$ and then both perform writes on the $\ms{head.next}$. 
The resulting schedule is trivially correct (both operations
return $\ms{true}$ so the schedule can some from a complete linearizable history).  
However, in the schedule, one of the operations, say $\lit{insert}(1)$,
overwrites the effect of the other one.  
Thus, if we extend the schedule with a complete execution of
$\lit{contains}(2)$, the only possible response it may give is
$\ms{false}$ which obviously does not produce a linearizable high-level history.  
%
\begin{figure*}[!h]
\scalebox{0.75}{
\input{figure1}}
 \caption{\small{
An observably incorrect schedule $\sigma$; % state of the list is empty; 
for succinctness, $R(h)$ and R(t) refers to reads of both \emph{val} and \emph{next} fields; $W(h)$ refers to write
on $head.next$}}\label{fig:ex1}%
\vspace{-0.35mm}
\end{figure*}
%
\begin{theorem}[Optimality]
\label{th:lrelaxed}
%Algorithm~\ref{alg:listver} 
The Versioned List implementation accepts all observably correct schedules. % with respect to $(\ms{LL},\ms{set})$.
\end{theorem}
%
\begin{proof}
%
Let $\sigma$ be any schedule of our concurrent implementation.
Recall that, for every update operation $\pi$ in $\sigma$, $\sigma|\pi$ is defined to be the subsequence
$\sigma|\pi$ consisting of the reads, writes and node creation events from the last
invocation of the function $\lit{waitfree-traversal}$ by $\pi$ in Lines~\ref{line:insert-start} and \ref{line:delete-start}; and
for every $\pi=\lit{contains}$ in $\sigma$, $\sigma|\pi$ is the subsequence
$\sigma|\pi$ consisting of the reads and writes on a node's \emph{val} and \emph{next} fields.

We prove that any schedule \emph{rejected} by our algorithm is  
not observably correct.
More precisely, we show that an operation restarts a fragment
of it execution (in Lines~\ref{line:insert-restart2}, \ref{line:remove-restart2}) 
only if extending it with a read or a write
on $\ms{next}$ or $\ms{val}$ fields would result in schedule that is
not observably correct.

We first observe that if a node is logically deleted
(Line~\ref{line:isdeleted}), then its next write renders the node
unreachable from the \ms{head} node (Line~\ref{line:delcommit}). 
Thus, an update operation $\pi$ partially restarts because of reading a logically
deleted node (Lines~\ref{line:insert-restart1},
or \ref{line:remove-restart1}) only if it is concurrent with a
\lit{remove} operation which, when completed would physically remove
the node addressed by $\pi$ at the end of its traversal. 
It is easy to see that regardless of what this operation $\pi$ is
($\lit{insert}(v)$ or $\lit{remove}(v)$), if we complete it in turn
and then extend the resulting schedule with $\lit{contains}(v)$, the
effect of $\pi$ will not be seen and the schedule will not be
linearizable.

Similarly, an update operation $\pi$ partially restarts in Lines~\ref{line:insert-restart2}, \ref{line:remove-restart2} 
after finishing its traversal phase, if
it fails in grabbing a lock on one of the nodes it is about to modify.
Thus, $\pi$ is concurrent with another update operating on the same node.  
Again, by completing both $\pi$ and the concurrent update, we obtain a
schedule in which one of the updates is ``lost'', so that its
extension with some $\lit{contains}(v)$ will not be linearizable.                 
%
% We prove that any schedule \emph{rejected} by our algorithm is  
% not observably correct.
% More precisely, we show that an operation restarts a fragment
% of it execution (in Lines~\ref{line:insert-restart2}, \ref{line:remove-restart2}) 
% only if extending it with a read or a write
% on $\ms{next}$ or $\ms{val}$ fields would result in schedule that is
% not observably correct.
% 
% We first observe that if a node is logically deleted
% (Line~\ref{line:isdeleted}), then its next write renders the node
% unreachable from the \ms{head} node (Line~\ref{line:delcommit}). 
% Thus, an update operation $\pi$ partially restarts because of reading a logically
% deleted node (Lines~\ref{line:insert-restart1},
% or \ref{line:remove-restart1}) only if it is concurrent with a
% \lit{remove} operation which, when completed would physically remove
% the node addressed by $\pi$ at the end of its traversal. 
% It is easy to see that regardless of what this operation $\pi$ is
% ($\lit{insert}(v)$ or $\lit{remove}(v)$), if we complete it in turn
% and then extend the resulting schedule with $\lit{contains}(v)$, the
% effect of $\pi$ will not be seen and the schedule will not be
% linearizable.
% 
% Similarly, an update operation $\pi$ partially restarts in Lines~\ref{line:insert-restart2}, \ref{line:remove-restart2}, or
% \ref{line:remove-restart3}, after finishing its traversal phase,  if
% it fails in grabbing a lock on one of the nodes it is about to modify.
% Thus, $\pi$ is concurrent with another update operating on the same node.  
% Again, by completing both $\pi$ and the concurrent update, we obtain a
% schedule in which one of the updates is ``lost'', so that its
% extension with some $\lit{contains}(v)$ will not be linearizable.                 
%
%
\end{proof}
%
%
% \subsection{Concurrency analysis of popular list-based set implementations}
% \label{sec:concur-list}
% %
% In this section,
Theorem~\ref{th:lrelaxed} shows that our implementation only rejects concurrent schedules that would result in
a violation of linearizability.
On the other hand, as Lemmas~\ref{lm:ll} and \ref{lm:hm} show, 
we can easily describe observably correct schedules that are rejected by the Lazy Linked list~\cite{HHL+05}
and Harris-Michael Linked list implementations~\cite{harris-set,michael-set}.
%


==> prel.tex <==
%!TEX root = paper-p.tex
\section{Preliminaries}
\label{sec:prel}
%
\myparagraph{Objects and implementations}
We consider a standard asynchronous shared-memory system, in which $n>1$
processes (or \emph{threads} of computation) $p_1,\ldots , p_n$ communicate by applying operations on
shared \emph{objects}. %\vincent{What is an operation?}
%
An object is an instance of an \emph{abstract data type} that
specifies the set of operations the object exports, the set of
responses the operations return, the set of states the object can
take, and the sequential specification that
stipulates the object's correct sequential behavior.  
%\vincent{Avoid "provided" here.}
% An \emph{abstract data type} $\tau$ is a tuple
% $(\Phi,\Gamma, Q, q_0, \delta)$ where
% $\Phi$ is a set of operations,
% $\Gamma$ is a set of responses, $Q$ is a set of states, $q_0\in Q$ is an
% initial state and 
% $\delta \subseteq Q\times \Phi \times Q\times \Gamma$ 
% is a transition relation that determines, for each state
% and each operation, the set of possible
% resulting states and produced responses~\cite{AFHHT07}. 
% Here, $(q,\pi,q',r) \in \delta$ implies that when
% an operation $\pi \in \Phi$ is applied on an object of type $\tau$
% in state $q$, the object may move to state $q'$ and return a response
% $r$. %\petr{we do not assume necessarily deterministic objects, right?}
To \emph{implement} a \emph{high-level} object from a set of shared
\emph{base} objects, processes follow an \emph{algorithm}, which is a
collection of deterministic state machines, one for each process. 
The algorithm assigns initial values to the base objects and processes
and specifies
the base-object operations a process must perform when it executes
every given operation. 
 To avoid confusion, we call operations on the base objects \emph{ primitives}. 
%We also say that an operation of an implemented object is performed
%and that a primitive is applied to a base object.
%A concurrent \emph{implementation} of an object type $\tau$ 
%provides a specific data-representation for the object   
%applying \emph{primitives} on
%shared \emph{base objects}, each of which is assigned an initial value and a set of algorithms $I_1(\tau),\ldots , I_n(\tau)$,
%one for each process.
%We assume that these primitives are deterministic.
A primitive is an atomic \emph{read}, \emph{write} or a \emph{read-modify-write (rmw)} instruction 
(\emph{e.g}, \emph{compare-and-swap (CAS)}) on a base object~\cite{Her91}.
% characterized by a pair of deterministic functions $\langle g,h \rangle$:
% given the current state of the base object, $g$ is an \emph{update function} that
% computes its state after the primitive is applied, while $h$ 
% is a \emph{response function} that specifies the outcome of the
% primitive returned to the process.
% % [[VG: RMW->rmw
% Special cases of rmw primitives are \emph{read} ($g$ leaves the state
% %]]
% unchanged and $h$ returns the state), \emph{write} ($g$ updates the
% state with its argument and $h$ returns $ok$) and \emph{compare-and-swap} (takes argument $\langle \ms{old},\ms{new} \rangle$ 
% and atomically updates the state of a base object to $\ms{new}$ and returns $\true$ \emph{iff} 
% its value prior to applying is equal to $\ms{old}$; otherwise it returns $\false$).   
%[[PK not needed?
%A rmw primitive is \emph{trivial} if it never changes the value of the
%base object to which it is applied.
%Otherwise, it is \emph{nontrivial}.
%\petr{Do we need the distinction trivial-nontrivial?}
%]]
%Throughout this paper, the term \emph{operation} refers to some
%high-level operation of the type and the term \emph{primitive} refers to actions on base objects.

% In a \emph{concurrent implementation} of an object type $\tau$,
% a process applying an operation $\pi \in \Phi$ is allowed to return a special response
% $\bot \not\in \Gamma$. In this case, we say that the corresponding high-level
% operation is \emph{aborted}. 

\myparagraph{Executions}
An \emph{event} of a process $p_i$ %(sometimes we say \emph{step} of $p_i$ \vincent{Why? can't we choose a single notation?})
is an invocation or response of an operation performed by $p_i$ on a
high-level object implementation, 
%\vincent{What does this 'or' separate?} 
%\vitaly{remind how rmw (g, h) works}
a \emph{rmw} primitive $\langle g,h \rangle$ applied by $p_i$ to a base object $b$
along with its response $r$ (we call it a \emph{rmw event} and write $(b, \langle g,h\rangle, r,i)$).
%\vincent{What is the difference between a primitive and an operation?}
%[[PK not sure we need this
%An event is \emph{trivial} (and resp. nontrivial) if it is the application of a trivial (and resp. nontrivial) primtive.
%]]
A \emph{configuration} specifies the value of each base object and 
the state of each process.
The \emph{initial configuration} is the configuration in which all 
base objects have their initial values and all processes are in their initial states.

An \emph{execution fragment} is a (finite or infinite) sequence of events.
An \emph{execution} of an implementation $I$ is an execution
fragment where, starting from the initial configuration, each event is
issued according to $I$ and each response of a rmw event $(b, \langle
g,h\rangle, r,i)$ matches the state of $b$ resulting from all
preceding events.
We assume that executions are \emph{well-formed}:
no process invokes a new high-level operation before
the previous high-level operation returns.

Let $\alpha|p_i$ denote the subsequence of an execution $\alpha$
restricted to the events of process $p_i$.
Executions $\alpha$ and $\alpha'$ are \emph{equivalent} if for every process
$p_i$, $\alpha|p_i=\alpha'|p_i$.
An operation $\pi$ \emph{precedes} another operation $\pi'$ in an execution
$\alpha$, 
denoted $\pi \rightarrow_{\alpha} \pi'$, 
if the response of $\pi$ occurs before the invocation of $\pi'$ in $\alpha$.
Two operations are \emph{concurrent} if neither precedes
the other. 
%An execution is \emph{rw-sequential} if every invocation of a read or write operation is immediately followed by a response event.
An execution is \emph{sequential} if it has no concurrent 
operations. 
An operation is \emph{complete} in $\alpha$ if the invocation event is
followed by a \emph{matching} response; otherwise, it is \emph{incomplete} in $\alpha$.
Execution $\alpha$ is \emph{complete} if every operation is complete in $\alpha$.

\myparagraph{High-level histories and linearizability}
A \emph{high-level history} $\tilde H$ of an execution $\alpha$ is the subsequence of $\alpha$ consisting of all
invocations and responses of %\emph{non-aborted} 
(high-level) operations.
%

%\begin{definition}
A complete high-level history $\tilde H$ is \emph{linearizable} with 
respect to an object type $\tau$ if there exists
a sequential high-level history $S$ equivalent to $\tilde H$ such that
(1) $\rightarrow_{\tilde H}\subseteq \rightarrow_S$ and
(2) \emph{$S$ is consistent with the sequential specification of type $\tau$}.
%\end{definition}
%
Now a high-level history $\tilde H$ is linearizable if it can be
\emph{completed} (by adding matching responses to a subset of
incomplete operations in $\tilde H$ and removing the rest)
to a linearizable high-level history~\cite{HW90,AW04}.
%

\myparagraph{Sequential implementations}
A \emph{sequential implementation} of an object type $\tau$ 
specifies, for each operation of $\tau$, a deterministic procedure that 
performs \emph{read} and \emph{write} primitives on a collection of base objects
that encode the state of the object, and returns a
response, so that the specification of $\tau$ is respected
in all sequential executions.   
%

Consider  the conventional \textsf{set} type exporting
$\lit{insert}$, $\lit{remove}$, and $\lit{contains}$ operations with
standard sequential semantics: $\lit{insert}(v)$
adds $v$ to the set and returns $\true$ if $v$ is not already there,
and returns $\false$ otherwise; $\lit{remove}(v)$ 
drops $v$ from the set and returns $\true$ if $v$ is there,
and returns $\false$ otherwise; and $ \lit{contains}(v)$ returns
$\true$ if and only if $v$ is in the set.
We consider the sequential implementation of the set type (denoted \LL) that uses a \emph{sorted linked list}. The exact specification and the list-based sequential
implementation of \textsf{set} are presented in the full version of the paper~\cite{arxiv-list}.


==> pseudocode-2.tex <==
%!TEX root = paper-p.tex
\begin{algorithm*}[!h]%
\caption{The versioned list-based set\label{alg:listver}}%
  \begin{algorithmic}[1]%
  	\begin{multicols}{2}%
  	{\size
	
	\Part{Shared variables}{
		\State node is a record with fields: \label{line:node-start}
		\State ~~~$\ms{val}$
		\State ~~~$\ms{next}$
		\State ~~~$\ms{deleted}$
		\State ~~~$\ms{vlock}$, a versioned lock: LSB is lock \label{line:vlock}
		
		\State ~~~$\ms{head.val} = -\infty$, $\ms{tail.val} = +\infty$
		\State ~~~$\ms{head.next} = \ms{tail}$
		\State ~~~$\ms{head.deleted} = \ms{tail.deleted} = \lit{false}$
		\State ~~~$\ms{head.vlock} = \ms{tail.vlock} = \tup{\ms{0}, \lit{false}}$ \label{line:node-end}
	}\EndPart

	\Statex
	
% ------------- contains ---------------
	\Part{$\lit{contains}(v)$}{			\Comment{wait-free contains}
		\State $\ms{curr} \gets \ms{head}$
		\While{$\ms{curr.val} < v$}
			\State $\ms{curr} \gets \ms{curr.next}$
		\EndWhile
		\State {\bf return} $(\ms{curr.val} = v \wedge \neg \ms{curr.deleted})$\label{line:linr}
	}\EndPart

	\Statex

% ------------- validate ---------------
	\Part{$\lit{validate}( \ms{prev}, \ms{curr})$}{
		\State $\ms{pVer} \gets \ms{prev.vlock}.\lit{getVersion}()$
                \label{line:validate-start}
		\If{$\ms{prev.deleted}$} {\bf return $\bot$} \label{line:check-prev} \EndIf 
		\If{$\ms{prev.next}\neq \ms{curr}$} {\bf return $\bot$} \EndIf
		%\State $\ms{curr} \gets \ms{prev.next}$
		\State {\bf return} $\ms{pVer}$ \label{line:validate-return} 
	}\EndPart

	\Statex

% ------------- traversal ---------------
	\Part{$\lit{waitfreeTraversal}(v,\ms{prev})$}{	\Comment{wait-free traversal}\label{line:traversal-start}
		\If{$\ms{prev.deleted}$} 
		  \State $\ms{prev} \gets \ms{head}$ 
		\EndIf
		\State $\ms{curr} \gets \ms{prev.next}$ \label{line:traverse:prev}
		\While{($\ms{curr.val}) < v$}		
		\State $\ms{prev} \gets \ms{curr}$	
		\State $\ms{curr} \gets \ms{curr.next}$
		\EndWhile
		\State {\bf return} $\ms{prev}$\label{line:traversal-end}
	}\EndPart
	\newpage

% ------------- insert ---------------
	\Part{$\lit{insert}(v)$}{
		\State $\ms{prev}\gets \ms{head}$
		\State $\tup{ \ms{prev},\ms{curr}} \gets \lit{waitfreeTraversal}(v,\ms{prev})$\label{line:insert-start}
		\If {$curr.deleted$} $\lit{goto}$ line~\ref{line:insert-start}
		\EndIf
		
		\If {$curr.val = v$} {\bf return} $\lit{false}$ 
		\EndIf
		\If{$(\ms{pVer} \gets \lit{validate}(\ms{prev},\ms{curr})) = \bot$}\label{line:insert-validate}
			\State $\lit{goto}$ line~\ref{line:insert-start}  \label{line:insert-restart1}
		\EndIf
		\State $\ms{newNode.val} \gets v$   \label{line:new-node}
		\State $\ms{newNode.next} \gets \ms{curr}$
		\If {$\neg prev.vlock.\lit{tryLockAtVersion}(\ms{pVer})$} \label{line:inslock} %\Comment{v.-lock}
			\State $\lit{goto}$ line~\ref{line:insert-start}\label{line:insert-restart2} \Comment{restart traversal}
		\EndIf
		\State $\ms{prev.next} \gets \ms{newNode}$\label{line:inscommit}
		%\State $\lit{write}(\ms{prev.next}, \ms{new})$\label{line:inscommit}
		\State $prev.vlock.\lit{unlockAndIncrementVersion()}$ \label{line:relinsert}
		\State {\bf return} $\lit{true}$
	}\EndPart

	\Statex

% ------------- remove ---------------
	\Part{$\lit{remove}(v)$}{
		\State $\ms{prev}\gets \ms{head}$
		\State $\tup{\ms{prev},\ms{curr}} \gets \lit{waitfreeTraversal}(v,\ms{prev})$\label{line:delete-start}
		
		\If {($\ms{curr.val} \neq v \vee \ms{curr.deleted}$)} {\bf return} $\lit{false}$
		%\If {$\ms{curr.val} \neq v$} {\bf return} $\lit{false}$ \Comment{v is not in the set}
		\EndIf
		\If{$(\ms{pVer} \gets \lit{validate}(\ms{prev},\ms{curr})) = \bot$}\label{line:delete-validate}
			\State $\lit{goto}$ line~\ref{line:delete-start} \Comment{validate failed: restart}\label{line:remove-restart1}
		\EndIf
		\If{$\neg prev.vlock.\lit{tryLockAtVersion}(\ms{pVer})$} \label{line:remlock} %\Comment{v.-lock}
			\State $\lit{goto}$ line~\ref{line:delete-start}	\label{line:remove-restart2} 
		\EndIf
\State $curr.vlock.\lit{lockAtCurrentVersion()}$ \Comment{spin lock}\label{line:spinlock} 
%		\If{$\neg \lit{cas}(\ms{curr.vlock}, \tup{\ms{cVer}, \lit{false}}, \tup{\ms{cVer}, \lit{true}})$} \Comment{vers. lock}
%			\State $\ms{prev.vlock} \gets \tup{\ms{pVer}, \lit{false}}$		\Comment{unlock w/o version change}
%			\State $\lit{goto}$ line~\ref{line:delete-validate}	\Comment{partially abort}\label{line:remove-restart3}
%		\EndIf
		\State $\ms{curr.deleted} \gets \lit{true}$ \Comment{logical delete}\label{line:isdeleted}
		\State $\ms{prev.next} \gets \ms{curr.next}$ \Comment{physical delete}\label{line:delcommit}
		%\State $\lit{write}(\ms{prev.next}, \ms{curr.next})$ \Comment{physical delete}\label{line:delcommit}
		\State $curr.vlock.\lit{unlockAndIncrementVersion()}$\label{line:curr-unlock}
		\State $prev.vlock.\lit{unlockAndIncrementVersion()}$\label{line:relremove}
		\State {\bf return} $\lit{true}$
	}\EndPart 
	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm*}


==> pseudocode-old.tex <==
%!TEX root = paper-p.tex
\begin{algorithm*}[ht]%
\caption{The versioned list-based set\label{alg:listver}}%
  \begin{algorithmic}[1]%
  	\begin{multicols}{2}%
  	{\size
	
	\Part{Shared variables}{
		\State node is a record with fields: \label{line:node-start}
		\State ~~~$\ms{val}$, its value
		\State ~~~$\ms{next}$, its reference to the next node in the list
		\State ~~~$\ms{deleted}$, a boolean indicating whether the node is 
		\State ~~~~~logically deleted
		\State ~~~$\ms{vlock}$, a versioned lock: counter whose least significant 
		\State ~~~~~bit is a lock \label{line:vlock}
		\State Initially the list contains only two nodes $\ms{head}$, $\ms{tail}$,
		\State ~~~$\ms{head.val} = -\infty$, $\ms{tail.val} = +\infty$
		\State ~~~$\ms{head.next} = \ms{tail}$
		\State ~~~$\ms{head.deleted} = \ms{tail.deleted} = \lit{false}$
		\State ~~~$\ms{head.vlock} = \ms{tail.vlock} = \tup{\ms{0}, \lit{false}}$ \label{line:node-end}
	}\EndPart

	\Statex
	
% ------------- contains ---------------
	\Part{$\lit{contains}(v)$}{			\Comment{wait-free contains}
		\State $\ms{curr} \gets \ms{head}$
		\While{$\ms{curr.val} < v$}
			\State $\ms{curr} \gets \ms{curr.next}$
		\EndWhile
		\State {\bf return} $(\ms{curr.val} = v \wedge \neg \ms{curr.deleted})$\label{line:linr}
	}\EndPart

	\Statex

% ------------- validate ---------------
	\Part{$\lit{validate}(v, \ms{prev})$}{
		\State $\ms{pVer} \gets \ms{prev.vlock}.\lit{getVersion}()$
                \Comment{return lock version}\label{line:validate-start}
		\If{$\ms{prev.deleted}$} {\bf return $\bot$} \Comment{full abort}\label{line:check-prev} \EndIf 
		\State $\ms{curr} \gets \ms{prev.next}$
%		\State $\ms{cVer} \gets \ms{curr}.\lit{getVersion}()$\label{line:get-cver1}
%		\If{$\ms{curr.deleted}$} 
%                   $\lit{goto}$ line~\ref{line:validate-start} \Comment{if curr deleted: partially abort}\label{line:validate-restart1} 
%                 \EndIf  
		\While{$\ms{curr.val} < v$}
			
%			\State $\ms{pVer} \gets \ms{cVer}$
			\State $\ms{pVer} \gets \ms{curr.vlock}.\lit{getVersion}()$
\If{$\ms{curr.deleted}$}  
                            $\lit{goto}$ line~\ref{line:validate-start}  \Comment{partial abort}\label{line:validate-restart2} 
                        \EndIf 
			\State $\ms{prev} \gets \ms{curr}$ \Comment{the above line checks prev.deleted}
			\State $\ms{curr} \gets \ms{curr.next}$ \Comment{same as reading prev.next}
		\EndWhile
		\State {\bf return} $\tup{\ms{prev}, \ms{pVer},\ms{curr}}$ \label{line:validate-return} 
	}\EndPart

	\newpage

% ------------- traversal ---------------
	\Part{$\lit{waitfreeTraversal}(v)$}{	\Comment{wait-free traversal used in updates}\label{line:traversal-start}
		\State $\ms{prev} \gets \ms{curr} \gets \ms{head}$
		\While{($\ms{curr.val}) < v$}		\Comment{until position is reached}
		\State $\ms{prev} \gets \ms{curr}$	\Comment{keep track of the previous node}
		\State $\ms{curr} \gets \ms{curr.next}$
		\EndWhile
		\State {\bf return} $\ms{prev}$\label{line:traversal-end}
	}\EndPart
	\Statex

% ------------- insert ---------------
	\Part{$\lit{insert}(v)$}{
		\State $prev \gets \lit{waitfreeTraversal}(v)$\label{line:insert-start}
		\If{$(\tup{\ms{prev}, \ms{pVer}, \ms{curr}} \gets \lit{validate}(v, \ms{prev})) = \bot$}\label{line:insert-validate}
			\State $\lit{goto}$ line~\ref{line:insert-start}  \Comment{full abort: restart from beginning}\label{line:insert-restart1}
		\EndIf
		\If {$curr.deleted$} $\lit{goto}$ line~\ref{line:insert-validate}
		\EndIf
		\If {$curr.val = v$} {\bf return} $\lit{false}$ \Comment{v already in the set}
		\EndIf
		\State $\ms{newNode.val} \gets v$   \Comment{allocate a new node with value $v$}\label{line:new-node}
		\State $\ms{newNode.next} \gets \ms{curr}$
		\If {$\neg prev.vlock.\lit{tryLockAtVersion}(\ms{pVer})$} \Comment{v.-lock}\label{line:inslock}
			\State $\lit{goto}$ line~\ref{line:insert-validate}\label{line:insert-restart2} \Comment{partially abort}
		\EndIf
		\State $\ms{prev.next} \gets \ms{newNode}$\label{line:inscommit}
		%\State $\lit{write}(\ms{prev.next}, \ms{new})$\label{line:inscommit}
		\State $prev.vlock.\lit{unlockAndIncrementVersion()}$ \label{line:relinsert}
		\State {\bf return} $\lit{true}$
	}\EndPart

	\Statex

% ------------- remove ---------------
	\Part{$\lit{remove}(v)$}{
		\State $\ms{prev} \gets \lit{waitfreeTraversal}(v)$\label{line:delete-start}
		\If{$(\tup{\ms{prev}, \ms{pVer}, \ms{curr}} \gets \lit{validate}(v, \ms{prev})) = \bot$}\label{line:delete-validate}
			\State $\lit{goto}$ line~\ref{line:delete-start} \Comment{full abort: restart from beginning}\label{line:remove-restart1}
		\EndIf
		\If {($\ms{curr.val} \neq v \vee \ms{curr.deleted}$)} {\bf return} $\lit{false}$
		%\If {$\ms{curr.val} \neq v$} {\bf return} $\lit{false}$ \Comment{v is not in the set}
		\EndIf
		\If{$\neg prev.vlock.\lit{tryLockAtVersion}(\ms{pVer})$} \Comment{v.-lock}\label{line:remlock}
			\State $\lit{goto}$ line~\ref{line:delete-validate}	\Comment{partially abort}\label{line:remove-restart2} 
		\EndIf
\State $curr.vlock.\lit{lockAtCurrentVersion()}$ \Comment{spin lock}\label{line:spinlock} 
%		\If{$\neg \lit{cas}(\ms{curr.vlock}, \tup{\ms{cVer}, \lit{false}}, \tup{\ms{cVer}, \lit{true}})$} \Comment{vers. lock}
%			\State $\ms{prev.vlock} \gets \tup{\ms{pVer}, \lit{false}}$		\Comment{unlock w/o version change}
%			\State $\lit{goto}$ line~\ref{line:delete-validate}	\Comment{partially abort}\label{line:remove-restart3}
%		\EndIf
		\State $\ms{curr.deleted} \gets \lit{true}$ \Comment{logical delete}\label{line:isdeleted}
		\State $\ms{prev.next} \gets \ms{curr.next}$ \Comment{physical delete}\label{line:delcommit}
		%\State $\lit{write}(\ms{prev.next}, \ms{curr.next})$ \Comment{physical delete}\label{line:delcommit}
		\State $curr.vlock.\lit{unlockAndIncrementVersion()}$\label{line:curr-unlock}
		\State $prev.vlock.\lit{unlockAndIncrementVersion()}$\label{line:relremove}
		\State {\bf return} $\lit{true}$
	}\EndPart 
	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm*}


==> related.tex <==
%!TEX root = paper-p.tex
\section{Related work}
\label{sec:related}
%
\noindent\textbf{List-based sets.}
Heller \emph{et al.}~\cite{HHL+05} proposed the Lazy Linked List algorithm,
with a variety of optimizations. % to the Lazy Linked List algorithms. 
In particular, 
they %tested the use of the runtime type identification mechanism and 
mentioned doing a validation prior to locking, and using a single lock within an $\lit{insert}$ operation.
%As we showed, 
One of the reasons why our implementation is faster than the Lazy Linked List is 
the use of a new \emph{versioned try-lock} mechanism
(hinted in~\cite{timebasedtm} for the TM context)  that
allows validating before acquiring the lock.
%without requiring to retrieve the reference of next nodes when traversing the list.

Harris~\cite{harris-set} proposed a non-blocking linked list algorithm
that 
%exploits a low order bit as a deletion mark to 
splits the removal of a node into two atomic steps: a logical deletion
that marks the node and a physical removal 
that unlinks the node from the structure.
Michael~\cite{michael-set} proposed advanced memory reclamation algorithms for Harris' algorithm.
In our implementation, we %did not discuss memory reclamation and 
rely on Java's garbage collector for memory reclamation~\cite{hotspot}. 
%We believe that our implementation could outperform Michael's variant for the same reason it 
%outperforms Harris' one because it does not 
%combine the logical deletion mark with the next pointer of a node but separates metadata 
%(logical deletion and versions) from the structural data (next and
%value fields). \petr{Did not get the last point... }

For variants of these list-based sets, we refer to the textbook of Herlihy and Shavit~\cite{HS08-book}.

Fomitchev and Ruppert~\cite{FR04} proposed a lock-free linked list where nodes have a backlink field that allows to backtrack 
in the list in case a conflict is detected instead of restarting 
from the beginning of the list. Its contains operation helps remove marked nodes from the list.  
Gibson and Gramoli~\cite{GG15} proposed a more efficient variant with the same amortized complexity, called the selfish linked list. It features a wait-free contains operation that does not help. We are not aware of any implementation in Java.

\vspace{1em}\noindent\textbf{Concurrency metrics.}
% 
%There is a long tradition of using 
Sets of accepted schedules are commonly used as a
metric of concurrency provided by a shared-memory
implementation.
For static database transactions, 
Kung and Papadimitriou~\cite{KP79} use the metric to 
capture the parallelism of a locking scheme.
%by the amount of 
%interleavings of operations it could accept without having to 
%reschedule them~\cite{KP79}. 
While acknowledging that the metric is theoretical, they 
insist that it may
have ``practical significance as
well, if the schedulers in question have relatively small
scheduling times as compared with waiting and execution
times.'' 

Herlihy~\cite{Her90} employed the metric from \cite{KP79} to compare various
optimistic and pessimistic synchronization techniques using
commutativity
%\emph{commutativity}~\cite{Wei88} 
of operations constituting high-level transactions.   
A synchronization technique is implicitly considered in~\cite{Her90} as highly
concurrent, namely ``optimal'',
if no other technique accepts more schedules. 
%Unlike~\cite{KP79,Her90}, 
By contrast, we focus here on a \emph{dynamic} model where the scheduler cannot 
use the prior knowledge of all the shared addresses to be accessed.

Optimal concurrency can also be seen as a variant of
\emph{permissiveness}, originally defined
for Transactional memory (TM)~\cite{GHS08-permissiveness}, but extended to the case of dynamic data structures
with general high-level sequential semantics.      

In the TM context, Gramoli \emph{et al}.~\cite{GHF10} defined a concurrency metric, the \emph{input
acceptance}, as the ratio of committed transactions over aborted
transactions for a given schedule. 
Unlike our metric which is defined independently of the synchronization technique used (like locks or TMs), 
input acceptance does not apply to lock-based programs.
%[[[\textbf{SR: I do not follow what is said here}]]
%
%
%
%
%


==> vlock-alg.tex <==
\begin{algorithm*}[!h]
\caption{The CAS-based implementation for the versioned try-lock}
\label{alg:vlock}
  \begin{algorithmic}[1]
  	\begin{multicols}{2}
  	{\size
	
	\Part{Private field}{
		\State $\ms{lockValue}$, an integer that supports CAS
		\State Initially $\ms{lockValue} = 0$
	}\EndPart

	\Statex

	
% ------------- getVersion ---------------
	\Part{$\lit{getVersion}()$}{ \Comment {only return even value}
		\State {\bf return} $\ms{lockValue}$.read() \& $1111...1110$ 
	}\EndPart

	\Statex

% ------------- tryLockAtVersion ---------------
	\Part{$\lit{tryLockAtVersion}(ver)$}{ \Comment {assuming ver is even}
		\State {\bf return} $\ms{lockValue}$.CAS($ver$, $ver+1$) 
	}\EndPart

	\newpage

% ------------- lockAtCurrentVersion ---------------
	\Part{$\lit{lockAtCurrentVersion}()$}{ 
		\State $\ms{success} \gets \lit{false}$
		
		\While{($\neg \ms{success}$)} \Comment {spin until lock}
		\State $\ms{ver} \gets$ $\lit{getVersion()}$
		\State $\ms{success} \gets \ms{lockValue}$.$\lit{tryLockAtVersion}$($ver$)
		\EndWhile
	}\EndPart
	\Statex

% ------------- unlockAndIncrementVersion ---------------
	\Part{$\lit{unlockAndIncrementVersion}()$}{ \Comment{assumed locked (odd)}
		\State $\ms{val} \gets \ms{lockValue}$.read()
		\State $\ms{lockValue}$.CAS($val$, $val+1$) \Comment{could use atomicSet}
	}\EndPart

	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm*}

